On Best-Response Dynamics in Potential Games

The paper studies the convergence properties of (continuous) best-response dynamics from game theory. Despite their fundamental role in game theory, best-response dynamics are poorly understood in many games of interest due to the discontinuous, set-valued nature of the best-response map. The paper focuses on elucidating several important properties of best-response dynamics in the class of multi-agent games known as potential games---a class of games with fundamental importance in multi-agent systems and distributed control. It is shown that in almost every potential game and for almost every initial condition, the best-response dynamics (i) have a unique solution, (ii) converge to pure-strategy Nash equilibria, and (iii) converge at an exponential rate.

==> finite_time_convergence.tex <==
\section{Finite Time Convergence to Mixed Equilibria}
Prove the following:
\begin{lemma} \label{lemma_finite_time_convergence}
Let $\Gamma$ be a non-degenerate potential game and let $x^*$ be a mixed strategy equilibrium. Assume $x(t)$ follows a FP process. The set of initial conditions such that $x(t) = x^*$ for some $t\in[0,\infty)$ has Lebesgue measure zero.\footnote{Note: Reword this later.}
\end{lemma}

%Let $H:X\rightarrow X$ be given by $H:= BR - x$.
%We wish to show that $D\dot H\leq c$. We have $D\dot H = \frac{d D\cdot H}{d \calL^n}\calL^n + S$. That the first part is bounded shouldn't be hard to show. We wish to show that $S=0$. In particular, $S$



==> inequalities.tex <==
\section{Potential Production Inequalities} \label{sec_inequalities}
In this section we prove two key inequalities (\eqref{equation_pot_inequality1_1} and \eqref{equation_pot_inequality2_1}) that are the backbone of our proof of Theorem \ref{thrm_main_result}.

We note that in proving Theorem \ref{thrm_main_result} there is a fundamental dichotomy between studying completely mixed equilibria and incompletely mixed equilibria.
Completely mixed equilibria lie in the interior of the strategy space. At these points the gradient of the potential function is zero and the Hessian is non-singular; local analysis of the dynamics is relatively easy. On the other hand, incompletely mixed equilibria necessarily lie on the boundary of $X$ and the potential function may have a nonzero gradient at these points.\footnote{We note that in games that are first-order non-degenerate, the gradient is always non-zero at incompletely mixed equilibria.} Analysis of the dynamics around these points is fundamentally more delicate.

In order to handle incompletely mixed equilibria we construct a nonlinear projection whose range is a lower dimensional game in which the image of the equilibrium under consideration is completely mixed. This allows us to handle both types of mixed equilibria in a unified manner.

\subsection{Projection to a Lower-Dimensional Game} \label{sec_diff_ineq_prelims}
Let $x^*$ be a mixed equilibrium.\footnote{We note that $x^*$ is assumed to be fixed throughout the section and many of the subsequently defined terms are implicitly dependent on $x^*$.} Let $C_i = \carr_i(x^*_i)$, where $x_i^*$ is the player-$i$ component of $x^*$, let $C=C_1\cup\cdots\cup C_N =\carr(x^*)$, and assume that $Y_i$ is ordered so that $\{y_i^1,\ldots,y_i^{\gamma_i}\} = C_i$.
Let $\gamma_i = |C_i|$, let $\tilde{N} :=\left|\big\{i\in\{1,\ldots,N\}:~\gamma_i \geq 2\big\}\right|$, and assume that the player set is ordered so that $\gamma_i \geq 2$ for $i=1,\ldots,\tilde{N}$.
%Under the assumed ordering, players $1,\ldots,\tilde{N}$ use mixed strategies at $x^*$ and the remaining players use pure strategies.
Since $x^*$ is assumed to be a mixed-strategy equilibrium, we have $\tilde{N} \geq 1$.
%so that at least one player uses a mixed strategy at $x^*$.


Given an $x\in X$, we will frequently use the decomposition $x=(x_p,x_m)$, where $x_m := (x_i^k)_{i=1,\ldots,\tilde{N},~k=1,\ldots,\gamma_i-1}$ and $x_p$ contains the remaining components of $x$.\footnote{The subscript in $x_m$ is suggestive of ``mixed-strategy components'' and the subscript in $x_p$ is suggestive of ``pure-strategy components''.} Let
$\gamma := \sum_{i=1}^N (\gamma_i-1).$
Recalling that $\kappa$ is the dimension of $X$ (see \eqref{def_kappa}), note that for $x\in X$ we have $x\in \R^\kappa$, $x_m\in\R^{\gamma}$, and $x_p\in \R^{\kappa-\gamma}$.
%Let $F_i^k$ be as defined in \eqref{def_F}, and let $F$ be as defined in \eqref{def2_F}. By definition we have

The set of joint pure strategies $Y$ may be expressed as an ordered set $Y=\{y^1,\ldots,y^K\}$ where each element $y^\tau\in Y$, $\tau\in\{1,\ldots,K\}$ is an $N$-tuple of strategies.
For each pure strategy $y^{\tau}\in Y$, $\tau=1,\ldots,K$, let $u^{\tau}$ denote the pure-strategy potential associated with playing $y^\tau$; that is, $u^\tau := u(y^\tau)$, where $u$ is the pure form of the potential function defined in Section \ref{sec_prelims}. A vector of \emph{potential coefficients} $u=(u^\tau)_{\tau=1}^K$ is an element of $\R^K$.

Given a vector of potential coefficients $u\in \R^K$ and a strategy $x\in X$,
%Using \eqref{eq_potential_expanded_form2}, define the function $F_i^k:X\times\R^K\to\R$ as
let\footnote{We note that the functions $F_i^k$ and $F$ defined here are identical to those defined in (12) and (13) of \cite{swenson2017regular}, and used extensively throughout \cite{swenson2017regular}.}
\begin{equation} \label{def_F}
F_i^k(x,u):= \frac{\partial U(x)}{\partial x_i^k},
\end{equation}
for $i=1,\ldots,\tilde{N},~k=1,\ldots,\gamma_i-1$, and let
%Let
%\begin{equation}\label{def2_F}
%F(x,u) := \left( F_i^k(x,u) \right)_{\substack{i=1,\ldots,\tilde{N}\\ k=1,\ldots,\gamma_i-1}}.
%\end{equation}
%
%
%
%Let $F_i^k(x,u)$ be as defined in \eqref{def_F}, and let\footnote{The function $F_i^k(x,u)$ is defined in Chapter \ref{chapter_nondegen_games} and an important property of $F_i^k(x,u)$ (regarding its behavior at equilibrium strategies) is derived in \eqref{eq_equilibrium_equation}. See the discussion surrounding \eqref{def_F}--\eqref{eq_equilibrium_equation} for more details.}
$$F(x,u) := \left( F_i^k(x,u)\right)_{\substack{i=1,\ldots,\tilde{N}\\ k=1,\ldots,\gamma_i-1}} =
\left( \frac{\partial U(x)}{\partial x_i^k}\right)_{\substack{i=1,\ldots,\tilde{N}\\ k=1,\ldots,\gamma_i-1}}.$$
%
Differentiating \eqref{eq_potential_expanded_form2} we see that at the equilibrium $x^*$ we have $\frac{\partial U(x^*)}{\partial x_i^k} = 0$ for $i=1,\ldots,\tilde{N}$, $k=1,\ldots,\gamma_i-1$ (see Lemma \ref{lemma_carrier_vs_gradient} in appendix), or equivalently,
%\begin{equation}
%F_i^k(x^*,u) = U(y_i^{k+1},x^*_{-i}) - U(y_i^{1},x^*_{-i}) = 0
%\end{equation}
%for $i=1,\ldots,\tilde{N},~ k=1,\ldots,\gamma_i-1$.
%By \eqref{eq_equilibrium_equation}, at the equilibrium $x^*$ we have
$$
F(x^*,u) = F(x^*_p,x^*_m,u) = 0.
$$

By Definition \ref{def_equilibria_nomenclature}, the (mixed) equilibrium $x^*$ is completely mixed if $\gamma=\kappa$, and is incompletely mixed otherwise.
Suppose $\gamma<\kappa$ so that $x^*$ is incompletely mixed. Let $\vJ(x) := D_{x_m}F(x_p,x_m,u)$ and note that by definition we have $\vJ(x^*) = \tilde{\vH}(x^*)$.

%It is our intention to use the implicit function theorem to show that there exists function $g:\calD(g)\rightarrow \R^{\gamma}$, $\calD(g)\subset\R^{\kappa-\gamma}$ such that $F(x_p,g(x_p),u)=0$ for $x_p$ in a neighborhood of $x^*_p$. Let $\vJ(x) := D_{x_m} F(x_m,x_p,u)$ be the Jacobian of $F$ taken with respect to $x_m$. We showed in \eqref{eq_deriv_F_equals_hessian} that  $\vJ(x) = \tilde{\vH}(x)$.
Since $\Gamma$ is assumed to be a non-degenerate game, $\vJ(x^*)$ is invertible. By the implicit function theorem, there exists a function $g:\calD(g)\rightarrow \R^{\gamma}$ such that $F(x_p,g(x_p),u)$ $ = 0$ for all $x_p$ in a neighborhood of $x^*_p$, where  $\calD(g)\subset \R^{\kappa-\gamma}$ denotes the domain of $g$, $x_p^*\in\calD(g)$, and $\calD(g)$ is open.

The graph of $g$ is given by
$$\mbox{Graph}(g):=\{x\in X :~ x=(x_p,x_m),~ x_p \in \mathcal{D}(g),~ x_m = g(x_p)\}.$$
Note that $\Gr(g)$ is a smooth manifold with Hausdorff dimension $(\kappa-\gamma)$ \cite{EvansGariepy}.
%This implies $\Gr(g)$ has a Hausdorff dimension of $(\kappa-\gamma)$ [cite or explain].
An intuitive interpretation of $\Gr(g)$ is given in Remark \ref{remark_g}.

If $\Gamma$ is a non-degenerate potential game then, using the multilinarity of $U$, we see that $\gamma \geq 2$ (see Lemma \ref{lemma_two_players_mixing} in appendix). This implies that
\begin{equation}\label{eq_graph_size}
\Gr(g) \mbox{ has Hausdorff dimension at most }  (\kappa-2).
\end{equation}

Let $\Omega:=\Omega_{C}$, where $\Omega_{C}$ is defined in \eqref{def_C_face},
%\{x\in X:~ x_i^k = 0, ~i=1,\ldots,N,~k\geq \gamma_i\}$
denote the face of $X$ containing $x^*$.
%\footnote{By the construction of $C$ we have $y_i^1\in C_i$, which implies that $T_i^1(x^*_i)>0$, which implies that the constraint $\sum_{k=1}^{K_i-1}x_i^k = 1$ is not active.} (If $x^*$ is completely mixed, then $\Omega=X$.)
Define the mapping $\tilde \calP:\calD(\tilde{\calP}) \rightarrow \Omega$, with domain $\calD(\tilde{\calP}) := \{x=(x_p,x_m)\in X:~ x_p\in\calD(g)\}$, as follows. If $x^*$ is completely mixed then let $\tilde \calP(x) := x$ be the identity. Otherwise, let
\begin{equation} \label{def_calPtilde_map}
\tilde \calP(x) := x^*+\left(x - (x_p,g(x_p)) \right).
\end{equation}
Let $\tilde \calP_i^k(x)$ be the $(i,k)$-th coordinate map of $\tilde \calP$, so that $\tilde \calP = (\tilde \calP_i^k)_{\substack{i=1,\ldots,N\\ k=1,\ldots,K_i-1}}$.
Following the definitions, it is simple to verify that for $x\in \mathcal{D}(\tilde \calP)$ we have $\tilde \calP_i^k(x) = 0$ for all $(i,k)$ with $k\geq \gamma_i$, and hence $\tilde \calP$ indeed maps into $\Omega$.
%Thus, the effect of $\tilde \calP$ is to project a strategy $x$ onto the face of $X$ in which $x^*$ resides.

Let $\tilde X_i := \{\tilde x_i\in \R^{\gamma_i-1}:~ \tilde x_i^k \geq 0, k=1,\ldots,\gamma_i-1,~\sum_{k=1}^{\gamma_i-1} \tilde x_i^k \leq 1 \}$, $i=1,\ldots,\tilde{N}$, and let $\tilde X := \tilde X_1\times\cdots\times \tilde X_{\tilde{N}}$.
Let $\calP:\calD(\calP)\rightarrow \tilde X$ with domain $\calD(\calP) = \calD(\tilde{\calP}) \subset X$ be given by
\begin{equation} \label{def_calP_map}
\calP := (\tilde \calP_i^k)_{i=1,\ldots,\tilde{N},~k=1,\ldots,\gamma_i-1}.
\end{equation}
Note that $\calP$ contains the components of $\tilde \calP$ not constrained to zero. As we will see in the following section, $\calP$ may be interpreted as a projection into a lower dimensional game in which $\calP(x^*)$ is a completely mixed equilibrium.

%For strategies $x$ in a neighborhood of $x^*$, this effectively results in a projection of $x$ into a lower dimensional game in which all players use completely mixed strategies.


\subsection{Inequalities}
Let $\tilde{U}:\tilde X \rightarrow \R$ be given by
$$
\tilde{U}(\tilde x) := U(x_p^*, \tilde x),
$$
where $x^* = (x_p^*,x_m^*)$ is the mixed equilibrium fixed in the beginning of the section.
Let $\tilde{\Gamma}$ be a potential game with player set $\{1,\ldots,\tilde{N}\}$, mixed-strategy space $\tilde X_i$, $i=1,\ldots,\tilde{N}$, and potential function $\tilde{U}$. By construction, $\calP(x^*)$ is a completely mixed equilibrium of $\tilde{\Gamma}$. Moreover, by the definition of a non-degenerate equilibrium, the Hessian of $\tilde{U}$ is invertible at $\calP(x^*)$.

%so that $\calP(x^*)$ is a completely mixed equilibrium of $\tilde{\Gamma}$.
We are interested in studying the projection $\calP(\vx(t))$ of a FP process into the lower dimensional game $\tilde{\Gamma}$.\footnote{In the lower dimensional game $\tilde{\Gamma}$, the dynamics of the projected process are not precisely fictitious play dynamics. However, the behave \emph{nearly} like fictitious play dynamics, which is what allows us to establish these inequalities.}
We wish to show that the following two inequalities hold:\\
(i) For $x$ in a neighborhood of $x^*$
\begin{equation}\label{equation_pot_inequality1_1}
\big\vert \tilde{U}(\calP(x^*)) - \tilde{U}(\calP(x)) \big\vert \leq c_1 d^2(\calP(x),\calP(x^*)),
\end{equation}
for some constant $c_1>0$.\\
(ii) Suppose $(\vx(t))_{t\geq 0}$ is a FP process. For $\vx(t)$ residing in a neighborhood of $x^*$
\begin{equation}\label{equation_pot_inequality2_1}
\frac{d}{dt} \tilde{U}(\calP(\vx(t))) \geq c_2 d(\calP(\vx(t)),\calP(x^*)),
\end{equation}
for some constant $c_2>0$.

The first inequality follows from Taylor's theorem and the fact that $\nabla \tilde{U}(\calP(x^*)) = 0$.
The following section is devoted to proving \eqref{equation_pot_inequality2_1}.\footnote{We note that when we write these inequalities, we mean they are satisfied in an integrated sense (e.g., as used in \eqref{eq_inf_time_pf_eq1}--\eqref{eq_inf_time_pf_eq2}). In this section, we treat all of these as pointwise inequalities. A rigorous argument could be constructed using the chain rule in Sobolev spaces (see, for example, \cite{MR2293955}).}

\subsection{Proving the Differential Inequality}
We begin with Lemma \ref{lemma_IR1} which shows---roughly speaking---that within the interior of the action space, the FP vector field approximates the gradient field of the potential function.

The following definitions are useful in the lemma.
For $B\subseteq X$, let $P_{X_i}(B) := \{x_i\in X_i:~ (x_i,x_{-i}) \in B \mbox{ for some } x_{-i} \in X_{-i}\}$ be the projection of $B$ onto $X_i$.
Given an $x_i\in X_i$, let
$$
d(x_i,\partial X_i) := \min\{x_i^1,\ldots,x_i^{K_i-1},1-\sum_{k=1}^{K_i-1} x_i^k\}
$$
denote the distance from $x_i$ to the boundary of $X_i$. Let
$$
d(P_{X_i}(B),\partial X_i) := \inf_{x_i\in P_{X_i}(B)} d(x_i,\partial X_i)
$$
denote the distance between the set $P_{X_i}(B)$ and the boundary of $X_i$.

Since we will eventually be interested in studying a lower-dimensional game derived from $\Gamma$, in the lemma we consider an alternative game $\hat{\Gamma}$ of arbitrary size.
\begin{lemma}\label{lemma_IR1}
Let $\hat{\Gamma}$ be a potential game with player set $\{1,\ldots,\hat{N}\}$, action sets $\hat{Y}_i$, $i=1,\ldots,\hat{N}$, with cardinality $\hat{K}_i:=|\hat{Y}_i|$, and potential function $\hat{U}$. Let $\hat{X}=\hat{X}_1\times\cdots\times \hat{X}_{\hat{N}}$ denote the mixed strategy space.
% Let $\{1,\ldots,\hat{N}\}$ denote the set of players, let $\hat{X}=\hat{X}_1\times\cdots\times \hat{X}_{\hat{N}}$ denote the mixed strategy space, and let $\hat{U}$ denote the potential function.

Let $B\subset \hat{X}$ and fix $i\in\{1,\ldots,\hat{N}\}$.
%and suppose that $d({P_{X_i}}(B),\partial X_i) > 0$.
Then for all $x\in B$ there holds
\begin{equation} \label{IR1_eq0}
z_i\cdot \nabla_{x_i} \hat{U}(x)\geq c \|\nabla_{x_i} \hat{U}(x)\|_1, \quad\quad \forall~ z_i\in \BR_i(x_{-i}) - x_i
\end{equation}
where the constant $c$ is given by $c = d(P_{X_i}(B),\partial \hat{X}_i)$.
\end{lemma}
\begin{proof}
Let $x\in B$. If $\|\nabla_{x_i}\hat{U}(x)\|_1=0$, then $\nabla_{x_i} \hat{U}(x)=0$, and the inequality is trivially satisfied. Suppose from now on that $\|\nabla_{x_i}\hat{U}(x)\|_1 >0$.

Without loss of generality, assume that $Y_i$ is ordered so that
\begin{equation}\label{IR1_eq4}
\actionione \in \BR_i(x_{-i}).
\end{equation}
Differentiating \eqref{eq_potential_expanded_form2} we find that\footnote{Note that the domain of (expected) potential function $\hat{U}$ may be trivially extended to an open neighborhood around $\hat{X}$ (see Section \ref{sec_prelims}). Using this extension we see that the derivative is well defined for $x$ lying on the boundary of $\hat{X}$.}
\begin{equation}\label{IR1_eq2}
\frac{\partial \hat{U}(x)}{\partial x_i^{k}} = \hat{U}(\actionikone,x_{-i}) - \hat{U}(\actionione,x_{-i}).
\end{equation}
Together with \eqref{IR1_eq4}, this implies that for $k=1,\ldots,\hat{K}_i-1$ we have
\begin{equation} \label{IR1_eq1}
\actionikone \in \BR_i(x_{-i}) \iff \frac{\partial \hat{U}(x)}{\partial x_i^k}=0.
\end{equation}
Using the multlinearity of $\hat{U}$ we see that if $\xi_i\in \BR_i(x_{-i})$ and $\xi_i^k > 0$ then $\actionikone \in \BR_i(x_{-i})$. But, by \eqref{IR1_eq1} this implies that if $\xi_i\in \BR_i(x_{-i})$ and $\xi_i^k > 0$ then $\frac{\partial \hat{U}(x)}{\partial x_i^k} = 0$.
Noting that any $\xi_i\in \BR_i(x_{-i})$ is necessarily coordinatewise nonnegative, this gives
\begin{align} \label{IR1_eq3}
(\xi_i - x_i)\cdot \nabla_{x_i} \hat{U}(x) = \underbrace{\sum_{k=1}^{\hat{K}_i-1} \xi_i^k \frac{\partial \hat{U}(x)}{\partial x_i^{k}}}_{=0} - \sum_{k=1}^{\hat{K}_i-1} x_i^k \frac{\partial \hat{U}(x)}{\partial x_i^{k}}, \quad\quad \xi_i\in \BR_i(x_{-i})
\end{align}
%for $\xi_i \in BR_i(x_{-i})$.
Since we assume $x\in B$, we have $x_i^k \geq d(P_{\hat{X}_i}(B),\partial \hat{X}_i)$, for all $k=1,\ldots,\hat{K}_i-1$.
Since we assume $y_i^1\in \BR_i(x_{-i})$, from \eqref{IR1_eq2} we get that $\frac{\partial \hat{U}(x)}{\partial x_i^{k}}\leq 0$ for all $k=1,\ldots,\hat{K}_i-1$. Substituting into \eqref{IR1_eq3}, this gives
\begin{equation}
(\xi_i - x_i)\cdot \nabla_{x_i} \hat{U}(x) \geq d(P_{\hat{X}_i}(B),\partial \hat{X}_i) \sum_{k=1}^{\hat{K}_i-1} \left(-\frac{\partial \hat{U}(x)}{\partial x_i^{k}}\right), \quad\quad \xi_i \in \BR_i(x_{-i}).
\end{equation}
But since $\frac{\partial \hat{U}(x)}{\partial x_i^{k}}\leq 0$ for all $k$ we have $\sum_{k=1}^{\hat{K}_i-1} \left(-\frac{\partial \hat{U}(x)}{\partial x_i^{k}}\right) = \|\nabla_{x_i}\hat{U}(x)\|_{1}$, and hence
$$
(\xi_i - x_i)\cdot \nabla_{x_i} \hat{U}(x) \geq d(P_{\hat{X}_i}(B),\partial \hat{X}_i) \|\nabla_{x_i}\hat{U}(x)\|_1, \quad\quad \xi_i \in \BR_i(x_{-i}),
$$
which is the desired result.
\end{proof}










\begin{remark} \label{remark_norm_equivalence}
Since the space $X_i$ in Lemma \ref{lemma_IR1} is finite dimensional, given any norm $\|\cdot\|$, there exists a constant $\tilde c>0$ such that
$$
z_i\cdot \nabla_{x_i} U(x)\geq c \|\nabla_{x_i} U(x)\|, \quad\quad ~ \forall ~z_i\in \BR_i(x_{-i})-x_i
$$
with $c = \tilde c d(P_{X_i}(B),\partial X_i)$.
\end{remark}

%%We are interested in studying convergence to $\Gr(g)$. We study this by projecting onto a reduced game consisting of only of mixing players and the free components $(x_i^k)_{i=1,\ldots,M,~k=1,\ldots,\gamma_i-1}$. In order to study the dynamics in terms of these components we define the following terms.
For each $x=(x_p,x_m)\in X$ near to $x^*$, the following lemma allows us to define an additional lower dimensional game $\Gamma_{x_p}$ associated with $x_p$ in which the best response set is closely related to the best response set for the original game $\Gamma$.
The lemma is a straightforward consequence of the definition of the best response correspondence and the continuity of $\nabla U$.
\begin{lemma} \label{lemma_IR4}
For $x$ in a neighborhood of $x^*$, the best response set satisfies
$$
\BR_i(x_{-i}) \subseteq \BR_i(x^*_{-i}),\quad \quad \forall ~i=1,\ldots,\tilde{N}.
$$
\end{lemma}


Given any $x = (x_p,x_m) \in X$ we define $\tilde U_{x_p}:\tilde X\rightarrow \R$ and $\BRtilde_{x_p,i}:\tilde X_{-i}\rightrightarrows \tilde X_i$ as follows. For $\tilde x \in \tilde X$ let
\begin{equation} \label{eq_V_tilde}
\tilde U_{x_p}(\tilde x) :=  U(x_p, \tilde x),
\end{equation}
and for $\tilde x_{-i} \in \tilde X_{-i}$ let
\begin{equation} \label{eq_BR_tilde}
\BRtilde_{x_p,i}(\tilde x_{-i}) := \arg\max_{\tilde{x}_i \in \tilde X_i} \tilde U_{x_p}(\tilde{x}_i,\tilde x_{-i})
\end{equation}


Let $\Gamma_{x_p}$ be the potential game with player set $\{1,\ldots,\tilde{N}\}$, mixed strategy space $\tilde X$ and potential function $\tilde U_{x_p}$. Note that since $U$ is continuous and $\tilde X$ is compact, $\tilde U_{x_p}$ converges uniformly to $\tilde U_{x_p^*} =: \tilde{U}$ as $x_p \rightarrow x_p^*$. In this sense the game $\Gamma_{x_p}$ can be seen as converging to $\tilde{\Gamma}$ as $x_p \rightarrow x_p^*$.
\begin{remark}\label{remark_g}
The function $g$ defined in Section \ref{sec_diff_ineq_prelims} admits the following interpretation.
Suppose we fix some $x_p = (x_i^k)_{i=1,\ldots,N,~k=\gamma_i,\ldots,K_i-1}$.
%Let $\Gamma_{x_p}$ be the game with player set $\{1,\ldots,\tilde{N}\}$, action set of player $i$ given by $\{y_i^1,\ldots,y_i^{\gamma_i}\} = \carr_i(x^*)$ and the utility function, identical for each player, given by $\tilde U_{x_p}$.
Then $g(x_p)$ is a completely mixed Nash equilibrium of $\Gamma_{x_p}$. Moreover, if we let $x_p\rightarrow x_p^*$, then the corresponding equilibrium of the reduced game $\Gamma_{x_p}$ converges to $x^*$, i.e., $(x_p,g(x_p)) \rightarrow (x_p^*,g(x_p^*)) = x^*$, precisely along $\Gr(g)$.
\end{remark}
\begin{remark} \label{remark_first_order_degeneracy}
Suppose $x^*$ is a first-order non-degenerate equilibrium. Using the multilinearity of $U$ we see that for any $x\in X$ we have $\carr_i(x_i) \subseteq \BR_i(x_{-i})$. By Remark \ref{remark_first_order_equivalent_condition}, at $x^*$ we have $\carr_i(x_i^*) = \BR_i(x_{-i}^*)$.
%a pure-strategy best response satisfies $y_i^k\in \BR_i(x_{-i}^*)$ if and only if $y_i^k\in \carr_i(x^*_i)$.
Due to the ordering we assumed on $Y_i$, this implies that
%$y_i^k\in \carr_i(x^*) \iff 1\leq k \leq \gamma_i$. Hence
$y_i^k \in \BR_i(x_{-i}^*) \iff 1\leq k\leq \gamma_i$. Moving to the $X$ domain, this means that if $\hat{x}_i \in \BR_i(x_{-i}^*)$, then $\hat{x}_i^k = 0$ for all $k=\gamma_i,\ldots,K_i-1$. By Lemma \ref{lemma_IR4}, this implies that for all $x$ in a neighborhood of $x^*$ and for $\hat{x}_i \in \BR_i(x_{-i})$ we have $(\hat{x}_i^k)_{k=\gamma_i}^{K_i-1} = 0$.
\end{remark}

The following lemma extends the result of Lemma \ref{lemma_IR1} so it applies in a useful way to the potential function $\tilde U$ under the projection $\calP$.
\begin{lemma} \label{lemma_IR5}
There exists a constant $c>0$ such that for all $x=(x_p,x_m)$ in a neighborhood of $x^*$ and all $\eta\in\R^{\gamma_i-1}$ with $\|\eta\|$ sufficiently small we have
$$
(z_i + \eta) \cdot \nabla_{x_i} \tilde{U}(\calP(x)) \geq c\|\nabla_{x_i} \tilde{U}(\calP( x))\|,
$$
for all $z_i \in \BRtilde_{i,x_p}([x_m]_{-i}) - [x_m]_i$, where $[x_m]_i := (x_i^k)_{k=1,\ldots,\gamma_i-1}$ refers to the player-$i$ component of $x_m$ and $[x_m]_{-i}$ contains the components of $x_m$ corresponding to the remaining players.
\end{lemma}
\begin{proof}
%If $\|\nabla_{x_i} \tilde{U}(\calP( x))\| = 0$ then $\nabla_{x_i} \tilde{U}(\calP(x))=0$ and the inequality is trivially satisfied. Assume henceforth that $\|\nabla_{x_i} \tilde{U}(\calP( x))\| > 0$.

By construction, the projection $\calP(x^*)$
%(see \eqref{def_calP_map})
maps $x^*$ into the interior of $\tilde X$.
Choose $\epsilon>0$ such that the ball $B(\calP(x^*),\epsilon)\subset \tilde{X}$ is separated by a positive distance from the boundary of $\tilde X$.
Applying Lemma \ref{lemma_IR1} (and Remark \ref{remark_norm_equivalence}) to the game $\Gamma_{x_p}$ we see that there exists a constant $c>0$ such that for any $x=(x_p,x_m)\in X$ with $x_m \in B(\calP(x^*),\epsilon)$ there holds
\begin{equation} \label{IR5_eq1}
z_i \cdot \nabla_{x_i} \tilde U_{x_p}(x_m) \geq 4c\|\nabla_{x_i} \tilde U_{x_p}(x_m)\|
\end{equation}
for all $z_i \in \BRtilde_{x_p,i}([x_m]_{-i}) - [x_m]_i$. Note that the constant in Lemma \ref{lemma_IR1} is only dependent on the distance from the set $B$ (in this case, $B(\calP(x^*),\epsilon)$) to the boundary of the strategy space (in this case, $\tilde{X}$), and is independent of the particular potential function under consideration---this permits the choice of $c>0$ in \eqref{IR5_eq1} that holds uniformly for all $x_p$.

By the continuity of $U$ and $\calP$ we have
\begin{equation} \label{IR5_eq2}
\bigg\|\frac{\nabla \tilde U_{x_p}(\calP(x))}{\|\nabla \tilde U_{x_p}(\calP(x))\|} -
\frac{\nabla \tilde{U}(\calP(x))}{\|\nabla \tilde{U}(\calP(x))\|}\bigg\| <
\frac{2c}{\sqrt{2}}
\end{equation}
and $\calP(x) \in B(x^*,\epsilon)$, for all $x$ in a sufficiently small neighborhood of $x^*$ and $x\not\in \Gr(g)$.
Note that $\mbox{diam}\, \tilde{X}_i := \max_{x_i,x_i' \in \tilde{X}_i} \|x_i - x_i'\| = \sqrt{2}$, and hence, $\|z_i\| \leq \sqrt{2}$ for any $z_i \in \BRtilde_{x_p,i}([x_m]_{-i}) - [x_m]_i$, $x_m\in \tilde{X}$.
%Since
%%$\|z_i\|\leq \sqrt{K_i-1}$,
%$\|z_i\| \leq 1$,
%this, along with \eqref{IR5_eq1} gives
Thus, \eqref{IR5_eq1} and \eqref{IR5_eq2} give
$$
z_i\cdot \nabla \tilde{U}(\calP(x)) \geq 2c\|\nabla \tilde{U}(\calP(x))\|,
$$
for all $z_i \in \BRtilde_{x_p,i}([x_m]_{-i}) - [x_m]_i$ and all $x$ in a neighborhood of $x^*$, $x\not\in \Gr(g)$. As long as $\|\eta\|\leq c$, the desired result holds for $x$ in a neighborhood of $x^*$, $x\not\in \Gr(g)$.
But $x\in\Gr(g) \implies \calP(x) = \calP(x^*) \implies \nabla_{x_i} \tilde{U}(\calP(x))=0$, in which case the inequality is trivially satisfied.
\end{proof}

Finally, the following lemma shows that the differential inequality \eqref{equation_pot_inequality2_1} holds.
\begin{lemma}\label{lemma_IR3}
Let $\Gamma$ be a non-degenerate potential game with mixed equilibrium $x^*$, and let $(\vx(t))_{t\geq 0}$ be a FP process. Then the inequality \eqref{equation_pot_inequality2_1} holds for $\vx(t)$ in a neighborhood of $x^*$.
\end{lemma}
\begin{proof}
Let
$$
\vP(x) := \left( \frac{\partial \tilde \calP_i^k}{\partial x_j^\ell } \right)_{\substack{i=1,\ldots,\tilde{N}, k=1,\ldots,\gamma_i-1\\ j=1,\ldots,N,~ \ell=\gamma_i,\ldots,K_i-1}}
$$
where the partial derivatives are evaluated at $x$.
%Let the coordinates of $\tilde P = (\tilde P_i^j)$ be ordered so that $
The Jacobian of $\tilde \calP$ evaluated at $x$ is given by
$$
\left( \frac{\partial \tilde \calP_i^k}{\partial x_j^\ell}\right)_{\substack{i,j=1,\ldots,N,\\ k,\ell=1,\ldots,K_i-1}} =
\begin{pmatrix}
I & ~ \vP(x)\\
0 & ~ 0
\end{pmatrix}.
$$
Using the chain rule we may express the time derivative of the potential along the path $\tilde \calP(\vx(t))$ as
$$
\frac{d}{dt} U(\tilde \calP(\vx(t))) = \nabla U(\tilde \calP(\vx(t)))
\begin{pmatrix}
I & ~ \vP(x)\\
0 & ~ 0
\end{pmatrix} \dot{x}
= \nabla_{x_m} U(\tilde \calP(\vx(t)))(\vI ~~\vP(x))\dot{x}.
$$
For $i=1,\ldots,\tilde{N}$, $k=1,\ldots,\gamma_i-1$ let $\eta_i^k(t) := \sum_{j=1}^{N}\sum_{\ell=\gamma_j}^{K_i-1} \frac{\partial \tilde \calP_i^k}{\partial x_j^\ell}\dot x_i^\ell$, let $\eta_i(t) := (\eta_i^k(t))_{k=1}^{\gamma_i-1}$, and let $\eta(t) = (\eta_i(t))_{i=1}^{\tilde{N}}$.
Multiplying out the right two terms above we get
\begin{equation} \label{IR3_eq1}
\frac{d}{dt}U(\tilde \calP(\vx(t))) = \nabla_{x_m} U(\tilde \calP(\vx(t))) \, (\dot{x}_m + \eta(t))
%\begin{pmatrix}
%& \dot x_1^1 + \eta_1^1(t)\\
%& \vdots\\
%& \dot x_1^{\gamma_1-1} + \eta_1^{\gamma_1-1}(t)\\
%& \vdots\\
%& \dot x_i^k + \eta_i^k(t)\\
%& \vdots\\
%& \dot x_{\tilde{N}}^{1} + \eta_{\tilde{N}}^1(t)\\
%& \vdots\\
%& \dot x_{\tilde{N}}^{\gamma_{\tilde{N}}-1} + \eta_{\tilde{N}}^{\gamma_{\tilde{N}}-1}(t)\\
%& 0\\
%& \vdots\\
%& 0
%\end{pmatrix}.
\end{equation}
By Lemma \ref{lemma_IR4} and Remark \ref{remark_first_order_degeneracy}, if we restrict $\vx(t)$ to a sufficiently small neighborhood of $x^*$ then for any $z_i = (z_i',z_i'') \in \BR_i(\vx_{-i}(t))$, $z_i'=(z_i^k)_{k=1}^{\gamma_i-1}$, $z_i''=(z_i^k)_{k=\gamma_i}^{K_i-1}$, we have $z_i' \in \BRtilde_{x_p,i}([x_m]_{-i})$ and $z_i'' = 0$. We note two important consequences of this:\\
(i) If we restrict $\vx(t)$ to a sufficiently small neighborhood of $x^*$ and note that \newline $U(\tilde \calP(\vx(t))) = \tilde{U}(\calP(\vx(t))$, then by \eqref{IR3_eq1} we have
\begin{align} \label{IR3_eq2}
\frac{d}{dt} \tilde{U}(\calP(\vx(t))) & =
\nabla \tilde{U}(\calP(\vx(t))) \cdot
\begin{pmatrix}
z_1(t) + \eta_1(t)\\
\vdots\\
z_{\tilde{N}}(t) + \eta_{\tilde{N}}(t)
\end{pmatrix}\\
\nonumber & = \sum_{i=1}^{\tilde{N}}\nabla_{x_i} \tilde{U}(\calP(\vx(t))) \cdot (z_i(t) + \eta_i(t)),
\end{align}
where $z_i(t) \in \BRtilde_{x_p(t),i}([x_m(t)]_{-i}) - [x_m(t)]_i$.\\
(ii) We may force $\max_{i=1,\ldots,\tilde{N}} \|\eta_i\|$ to be arbitrarily small by restricting $\vx(t)$ to a neighborhood of $x^*$.

Consequence (i) follows readily by using the definition of FP \eqref{def_FP_autonomous}. To show consequence (ii), note that by \eqref{def_FP_autonomous} we have $\dot{\vx}_i^k = z_i^k - x_i^k$ for all $i=1,\ldots,N$, $k=1,\ldots,K_i$, for some $z_i \in \BR_i(x_{-i})$. But, for $x$ in a neighborhood of $x^*$ and $k\geq \gamma_i$, we have shown above that $z_i^k = 0$, and hence $\dot{x}_i^k = -x_i^k$.\footnote{We note that this particular step depends crucially on the assumption of first-order non-degeneracy (see Remark \ref{remark_first_order_degeneracy}).} Due the ordering we assumed for $Y_i$, we have $[x^*]_i^k = 0$ for any $(i,k)$ such that $k\geq \gamma_i$. Hence, $x_i^k \rightarrow 0$ as $x\rightarrow x^*$, for any $(i,k)$ such that $k\geq \gamma_i$.

Furthermore, there exists a $c>0$ such that $|\frac{\partial \tilde \calP_i^k(x)}{\partial x_j^\ell}| < c$, $i=1,\ldots,\tilde{N}$, $k=1,\ldots,\gamma_i-1$, $j=1,\ldots,N$, $\ell\geq \gamma_j$ uniformly for $x$ in a neighborhood of $x^*$ (see Lemma \ref{lemma_g_derivative_finite} in appendix).
%there exists a $c>0$ such that $|\frac{\partial \tilde \calP_i^k(x)}{\partial x_j^\ell}| < c$, $i=1,\ldots,N$, $k\geq \gamma_i$ for $x$ in a neighborhood of $x^*$ (see Lemma \ref{lemma_g_derivative_finite} in appendix).
By the definition of $\eta_i$, this implies that $\max_{i=1,\ldots,\tilde{N}} \|\eta_i\|$ may be made arbitrarily small by restricting $\vx(t)$ to a sufficiently small neighborhood of $x^*$.

Now, let $\vx(t)$ be restricted to a sufficiently small neighborhood of $x^*$ so that $\|\eta_i(t)\|$ is small enough to apply Lemma \ref{lemma_IR5} for each $i$. Applying Lemma \ref{lemma_IR5} to \eqref{IR3_eq2} we get
$
\frac{d}{dt} \tilde{U}(\calP(\vx(t))) \geq \sum_{i=1}^{\tilde{N}} c \|\nabla_{x_i} \tilde{U}(\calP(\vx(t)))\|
$
for $\vx(t)$ in a neighborhood of $x^*$. By the equivalence of finite-dimensional norms, there exists a constant $c_1$ such that $\frac{d}{dt} \tilde{U}(\calP(\vx(t))) \geq  c_1\|\nabla \tilde{U}(\calP(\vx(t)))\|$
for $\vx(t)$ in a neighborhood of $x^*$.


Since $\Gamma$ is assumed to be (second-order) non-degenerate, $\calP(x^*)$ is a non-degenerate critical point of $\tilde U$. By Lemma \ref{lemma_gradient_inequality_apx} (see appendix) there exists a constant $c_2$ such that
$c_1\|\nabla \tilde{U}(\tilde x)\| \geq c_2d(\tilde x,\calP(x^*))$ for all $\tilde x\in \tilde X$ in a neighborhood of $\calP(x^*)$.
%Here, $d$ is a metric on $X$ but the inequality is only guaranteed to hold for $\tilde x\in \tilde X$.
Since $\calP$ is continuous we have
$
\frac{d}{dt} \tilde{U}(\calP(\vx(t))) \geq c_2 d(\calP(\vx(t)),\calP(x^*)),
$
for $\vx(t)$ in a neighborhood of $x^*$.
\end{proof}
%\begin{remark}
%Note that Lemma \ref{lemma_IR5} together with \eqref{IR3_eq2} implies that $\frac{d}{dt} \tilde U(\calP(x(t))) \geq 0$ in a neighborhood of $x^*$.
%\end{remark}


==> introduction-Copy.tex <==
\section{Introduction} \label{sec_intro}
A Nash equilibrium (NE) is a solution concept for multi-player games in which no player can unilaterally improve their personal utility.
%Formally, a NE is defined as the fixed point of the best response mapping---that is, a strategy $x^*$ is said to be a NE if
Formally, a Nash equilibrium is defined as a fixed point of the best response mapping---that is, a strategy $x^*$ is said to be a NE if
$$
x^* \in \BR(x^*),
$$
where BR denotes the best response mapping (see Section \ref{sec_prelims} for a formal definition).

A question of fundamental interest is, given the opportunity to interact, how might a group of players adaptively learn to play a NE strategy over time?
In response, it is natural to consider the dynamical system induced by the best response mapping itself:
\begin{equation} \label{def_FP_autonomous}
\dot{\vx} \in \BR(\vx) - \vx.
\end{equation}
We refer to this learning procedure as the \emph{best response dynamics} \cite{gilboa1991social,matsui1992best,hofbauer1995stability,hopkins1999note,cortes2015self}. By definition, the set of NE coincide with the equilibrium points of these dynamics.
%Furthermore, intuition suggests that NE \emph{ought} to be attractors.

Best response adjustment processes in the spirit of \eqref{def_FP_autonomous} are ubiquitous throughout game theory. For example, the discrete-time learning process known as \emph{fictitious play} (FP) is a canonical algorithm which serves as a prototype for many other game-theoretic learning algorithms. FP is merely an Euler discretization of \eqref{def_FP_autonomous}.\footnote{In fact, many authors prefer to refer to \eqref{def_FP_autonomous} as \emph{continuous-time fictitious play} rather than best response dynamics \cite{harris1998rate,benaim2005stochastic,
leslie2006generalised,krishna1998convergence}.} In some algorithms the relationship is less direct--for example, \cite{leslie2006generalised} gives a payoff-based actor-critic algorithm in which players tend with high probability to pick best response actions---the underlying dynamics are governed by the differential inclusion \eqref{def_FP_autonomous}. The story is similar with many other learning processes which rely on underlying best response dynamics (e.g., \cite{coucheney2014penalty} [cite others]). The connections between discretized, perturbed, and possibly noisy, best-response based learning procedures and \eqref{def_FP_autonomous} can be made rigorous using the framework of stochastic approximations \cite{benaim2005stochastic}.

Despite the ubiquity of best-response-based learning algorithms, there is much we do not understand about the best response dynamics \eqref{def_FP_autonomous} in many important classes of games. In this paper our focus will be on elucidating several fundamental properties of \eqref{def_FP_autonomous} in the important class of multi-agent games known as \emph{potential games} \cite{Mond96}.

In a potential game, there exists an underlying potential function which all players implicitly seek to maximize. Such games are fundamentally cooperative in nature (all players benefit by maximizing the potential),
and have many important applications in engineering and economics \cite{marden2009cooperative,Mond96}. Along with so called \emph{harmonic games} (which are fundamentally adversarial in nature), potential games may be seen as one of the basic building blocks of general $N$-player games \cite{candogan-potential-decomposition}.

In the class of potential games, there are several fundamental properties of \eqref{def_FP_autonomous} that are not well understood. For example:
\begin{itemize}
\item It is known that solutions of \eqref{def_FP_autonomous} may not always be unique. However, in practice, one observes that in potential games, solutions often tend to be unique. The question thus arises: Can uniqueness of solutions of FP in potential games be demonstrated in some weaker sense (e.g., solutions are unique from almost every initial condition)?
\item It has been conjectured (and is generally believed to be true) that the rate of convergence of FP is exponential in potential games (\cite{harris1998rate}, Conjecture 25). However, no formal convergence rate estimates have been given. 
\end{itemize}


Underlying both of these issues is a single common problem. The set of NE may be subdivided into pure-strategy (deterministic) NE and mixed-strategy (probabilistic) NE. Mixed-strategy NE can be problematic for a number of reasons \cite{jordan1993}. Since \eqref{def_FP_autonomous} is a differential inclusion, trajectories of \eqref{def_FP_autonomous} can reach a mixed equilibrium in finite time. Once at a mixed equilibrium, a solution curve can rest there for an arbitrary length of time before moving elsewhere. This is the fundamental cause of non-uniqueness of solutions, and makes it impossible to establish general convergence rate estimates. 
%Moreover, it is important to note that since \eqref{def_FP_autonomous} is a differential inclusion, trajectories can reach mixed equilibria in finite time, at which point they loose uniqueness.
%Thus, it is of critical importance to understand when BR dynamics converge to mixed equilibria. 

From a less theoretical viewpoint, mixed equilibria also tend to be inherently problematic as solution concept in engineering applications since they are nondeterministic, have suboptimal expected utility, and do not always have clear physical meaning \cite{arslan2007autonomous}. Consequently, practitioners often prefer algorithms that
%preference is often given to algorithms that 
are guaranteed to converge to a pure-strategy NE \cite{marden-payoff,marden2009overcoming,arslan2007autonomous,li2013designing}.

%It is known that BR dynamics \emph{can} converge to mixed equilibria in potential games.
It has been speculated that convergence of BR dynamics to mixed equilibria should be rare in potential games \cite{krishna1998convergence,hofbauer1995stability,arslan2007autonomous}. Nevertheless, this issue is not well understood and there have been no formal results along these lines. 

In this paper we attempt to shed some light on these issues. Informally speaking, we will show that (i) BR dynamics almost never converge to mixed equilibria in potential games, (ii) solutions of \eqref{def_FP_autonomous} are almost always unique in potential games, and (iii) the rate of convergence of \eqref{def_FP_autonomous} is almost always exponential in potential games.

%\item  The set of NE may be subdivided into pure-strategy (deterministic) NE and mixed-strategy (probabilistic) NE.
%    Mixed-strategy NE can be problematic for a number of reasons \cite{jordan1993}.
%    In engineering applications involving potential games, mixed-strategy NE can be undesirable since they are nondeterministic, have suboptimal expected utility,    and do not always have clear physical meaning \cite{arslan2007autonomous}. Consequently, in applications, preference is often given to algorithms that are guaranteed to converge to a pure-strategy NE \cite{marden-payoff,marden2009overcoming,arslan2007autonomous,li2013designing}.
%    At a more fundamental level, mixed equilibria are highly problematic because they cause non-uniqueness of solutions and can make it impossible to establish general convergence rate estimates.
%    It is known that the BR dynamics \emph{can} converge to mixed strategy equilibria in potential games. However, it is generally believed that convergence of BR dynamics to mixed equilibria is an exception occurrence (e.g., \cite{krishna1998convergence,hofbauer1995stability,arslan2007autonomous}). Nevertheless, no such results have been shown.
%\end{enumerate}

The study of these issues is particularly challenging since once can easily construct counterexamples of potential games where BR dynamics behave poorly. As a first step in addressing these issues, in a companion paper \cite{swenson2017regular} we show that almost every potential game is regular in the sense introduced by Harsanyi \cite{harsanyi1973oddness}. In regular games, all equilibria are highly robust and relatively easy to analyze. Furthermore, as we will see below, regular games are ideally suited to studying best response dynamics.


%As noted in item 3 above, mixed equilibria cause non-uniqueness and make it impossible to establish general convergence rate estimates. 
The linchpin in addressing all of the issues noted above is gaining a rigorous understanding the question of convergence to mixed equilibria. The main result of the paper is the following.
\begin{theorem} \label{thrm_main_result}
Suppose $\Gamma$ is a regular potential game. Then from almost every initial condition, the BR dynamics \eqref{def_FP_autonomous} converge to a pure-strategy equilibrium. 
\end{theorem}
We emphasize that since almost every potential game is regular \cite{swenson2017regular}, this result implies generic convergence to pure NE in \emph{almost every} potential game.
%We note that a related result for two-player games has been shown in \cite{krishna1998convergence}, where it was demonstrated that FP almost never converges cyclically to a mixed-strategy equilibrium in which both players use more than two pure-strategies. In this paper we focus on $N$-player potential games and we show that, in such games, convergence to mixed equilibria is generically impossible.
As a byproduct of the proof of Theorem \ref{thrm_main_result} we will get the following result regarding uniqueness of solutions.
\begin{proposition}
Suppose $\Gamma$ is a regular potential game. Then solutions of \eqref{def_FP_autonomous} are unique for almost every initial condition. 
\end{proposition}
Finally, as a simple application of Theorem \ref{thrm_main_result} we will prove the following result. 
\begin{theorem} \label{thrm_conv_rate}
Suppose $\Gamma$ is a regular potential game. Then for almost every initial condition, best response dynamics converge to the set of NE at an exponential rate.
\end{theorem}
We remark that this resolves the Harris conjecture (\cite{harris1998rate}, Conjecture 25) on the rate of convergence of continuous-time fictitious play. 

The remainder of the paper is organized as follows. In Sections \ref{sec_proof_strategy}--\ref{sec_comparison} we outline our strategy for proving Theorem \ref{thrm_main_result} and compare with classical techniques.  Section \ref{sec_prelims} sets up notation and gives a simple example illustrating the fundamental problems arising in best response dynamics in potential games.
Section \ref{sec_reg_games} introduces regular potential games.
Section \ref{sec_inequalities} establishes the two key inequalities used to prove Theorem \ref{thrm_main_result}. Section \ref{sec_proof_main_result} gives the proof of Theorem \ref{thrm_main_result}. Finally, Section ?? proves Theorem \ref{thrm_conv_rate} as a simple consequence of Theorem \ref{thrm_main_result}.

\subsection{Proof Strategy} \label{sec_proof_strategy}
The basic strategy is to leverage two noteworthy properties satisfied in almost every potential game:\\
\begin{enumerate}
\item  The FP vector field cannot concentrate mass in finite time, meaning it cannot map a set of positive (Lebesgue) measure to a set of zero measure in finite time (see Section \ref{sec_finite_time_convergence}).\\
\item  In a neighborhood of an \emph{interior} Nash equilibrium (i.e., a \emph{completely mixed equilibrium}), the magnitude of the time derivative of the potential along paths grows linearly in the distance to the Nash equilibrium, while the value of the potential varies only quadratically; that is,
\[
\frac{d}{dt} U(\vx(t)) \geq d(\vx(t),x^*) \geq \sqrt{|U(\vx(t)) - U(x^*)|},
\]
where $U$ denotes the potential function and $x^*$ is the equilibrium point.\\
\end{enumerate}

Using Markov's inequality, property 2 immediately implies that if a path converges to an interior NE then it must do so in finite time (see Section \ref{sec_infinite_time_conv}). Hence, properties 1 and 2 together imply that the set of points from which FP converges to an interior NE must have Lebesgue measure zero.
 %(See Section \ref{sec_proof_main_result} for more details.)

In order to handle mixed NE that are \emph{not} in the interior of the strategy space (i.e., \emph{incompletely mixed equilibria}), we consider a projection that maps incompletely mixed equilibria to the \emph{interior} of the strategy space of a lower dimensional game.
Using the techniques described above we are then able to handle completely and incompletely mixed equilibria in a unified manner.

In particular, we see that the set of points from which FP converges to the set of mixed-strategy NE has Lebesgue measure zero. Since any FP path must converge to a NE \cite{benaim2005stochastic}, this implies Theorem \ref{thrm_main_result}.

Properties 1 and 2 hold as long the equilibrium $x^*$ is regular. In a companion paper we show that, in almost all potential games, all equilibria are regular (see Theorem \ref{thrm_reg_pot_games} below).

%Section \ref{sec_nondegenerate_games} uses techniques from \cite{harsanyi1973oddness}\footnote{NOTE: I was confused what paper you meant to reference here. Did you mean Harsanyi?} to prove that these conditions hold in almost all potential games.



\subsection{Comparison with Classical Techniques} \label{sec_comparison}

Given a classical ODE, one can prove that an equilibrium point may only be reached from a set of measure zero by studying the linearized dynamics at the equilibrium point.
%In particular, given some equilibrium point, consider the linearization of the ODE near the equilibrium point.
Assuming all eigenvalues associated with the linearized system are non-zero, the dimension of the stable manifold (i.e., the set of initial conditions from which the equilibrium can be reached) is equal to the dimension of the stable eigenspace of the linearized system \cite{Chicone_ODE}. Hence, to prove that an equilibrium can only be reached from a set of measure zero, it is sufficient to prove that at least one eigenvalue of the linearized system lies in the right half plane.

In FP, the vector field is discontinuous---hence, it is not possible to linearize around an equilibrium point, and such classical techniques cannot be directly applied.
%However, one may note that FP paths do tend to climb the potential function.
However, the gradient field of the potential function may be seen as an approximation of the FP vector field (see Lemma \ref{lemma_IR1}).
%In particular, it can be shown that the direction of the FP vector field approximately coincides with the direction of the gradient field of the potential function (see Lemma \ref{lemma_IR1}).
Unlike the FP vector field, the gradient field of the potential function \emph{can} be linearized. In a non-degenerate game, any completely mixed-strategy NE is a non-degenerate saddle point of the potential function. Hence, at least one eigenvalue of the linearized gradient system must lie in the right-half plane. This implies that, for the gradient dynamics of the potential function, the stable manifold associated with an equilibrium point has dimension at most $\kappa-1$, where $\kappa$ is the dimension of the strategy space.

Since the FP vector field approximates the gradient field of the potential function, intuition suggests that for FP dynamics, each mixed equilibrium should also admit a similar low-dimensional stable manifold.

While this provides an intuitive explanation for why one might expect Theorem \ref{thrm_main_result} to hold, we did not use any such linearization arguments in the proof of this result. We found that studying the rate of potential production near mixed equilibria (e.g., as discussed in the ``proof strategy'' section above) led to shorter and simpler proofs.
%However, we hypothesize that an alternate proof of Theorem \ref{thrm_main_result} could be obtained by considering smooth approximations to FP and linearizing near mixed-strategy equilibria.





